Graph-based keyword search in heterogeneous data sources

Data journalism is the field of investigative journalism which focuses on digital data by treating them as first-class citizens. Following the trends in human activity, which leaves strong digital traces, data journalism becomes increasingly important. However, as the number and the diversity of data sources increase, heterogeneous data models with different structure, or even no structure at all, need to be considered in query answering. Inspired by our collaboration with Le Monde, a leading French newspaper, we designed a novel query algorithm for exploiting such heterogeneous corpora through keyword search. We model our underlying data as graphs and, given a set of search terms, our algorithm nds links between them within and across the heterogeneous datasets included in the graph. We draw inspiration from prior work on keyword search in structured and unstructured data, which we extend with the data heterogeneity dimension, which makes the keyword search problem computationally harder. We implement our algorithm and we evaluate its performance using synthetic and real-world datasets.

==> approach.tex <==
\section{Building and storing the integrated graph}
\label{sec:dsa}
We now explain how we compute and store the elements of our graph, in particular sameAs edges which enable interconnecting datasets (Section~\ref{sec:equiv-nodes}), and entities we extract to enrich the graph (Section~\ref{sec:ie-approach}). 
%which are progressively filled with information\HG{could we call this metadata instead of information? information seems too vague} \IM{Ce sont des données, pas des méta données... et j'ai raccourci.}, as new datasets are {\em registered} (pre-processed) by our system; together, these data structures {\em implement the $G$ information essentially needed in order to answer queries efficiently}. 

% \vspace{-2mm}
%\mysubsection{Text index}
%\label{sec:index}
\mysubsection{Basic data structures} 
\label{sec:basicdatastructures}

\noindent\textbf{Nodes and edges} To each node $n\in G$, we associate ($i$)~a type (whether it stands for a dataset, an entity, a literal, a number, an URI etc.), and ($ii$)~a globally unique ID. These are stored in a relation $N(ID, type, \lambda)$ which also stores for each node $n$ its label $\lambda(n)$. Similarly, we store edges in a collection $E(ID, n_1.ID, n_2.ID, \lambda, c)$ where $n_1.ID,n_2.ID$ are the identifiers of the nodes defining the edge, $\lambda$ is its label and $c$ is its confidence between $0$ and $1$.

\noindent\textbf{Index} We build an {\em inverted index} accounting for the presence of (stemmed) keywords in our dataset. Specifically, the index $I(ID, kwd)$ associates a keyword  $w\in W$ with the IDs of the $G$ nodes (or edges) where it appears\footnote{Each index entry also contains an attribute which states whether $ID$ refers to a node or edge. For simplicity, we omit this attribute from our discussion.}. Following a common optimization in information retrieval systems, we only index noun words from text, based on the observation that non-noun words (e.g., verbs, pronouns etc.) are pretty common and may appear in many (text) datasets without this corresponding to a data connection. We %apply a few simple extraction rules to obtain e.g. from URIs some indexable elements, e.g., from https://www.lemonde.fr/economie/article/2019/01/14/produits-invendus-detruits-par-amazon-brune-poirson-annonce-une-loi\_5408701\_3234.html we would extract: ``Amazon'', ``Brune'', ``Poirson''.
also decompose URIs based on the separators present therein, and index the domain names as well as any nouns recognized in the URIs, as keywords associated to an URI node.

For instance, in our example dataset (Figure~\ref{fig:example-graph}), the index contains entries for ``I. Balkany'', ``Morocco'', ``Africa'', ``Areva'' etc. 
% \begin{itemize}
% \item  if the label is a text (occurring in a plain text, or as a string in JSON, relational or RDF data), we remove punctuation, and apply syntactic analysis to identify the nouns; they are stemmed, then each noun is indexed. The reason why we remove non-noun words is a heuristic, based on the observation that non-noun words (e.g., verbs, pronouns etc.) are pretty common and may appear across texts without this corresponding to a data connection; 
% \item if the label is an URI, we currently only use the domain as word; we obtain it as the text comprised after the {\em http://} or {\em https://} prefix, and the first slash sign following it. This is a conservative approach; one could have also extracted more words by separating the URIs according to signs such as /, \# etc., then applying some syntactic analysis to keep the nouns among the words thus obtained. 
% \end{itemize}

\subsection{More details on graph construction (aka data source registration)} \label{sec:loading-details}
The registration process goes over each source documents sequentially. 
Each documents is traversed generating all its nodes and edges; then, they are stored persistently or in memory ``within'' the data source object. The traversal process enumerates edges from the sources, and for each edge, that is not already part of the graph, we add it and proceed similarly with its source and target nodes. When a node is newly added to the graph, it undergoes an indexing process detailed below. The parameter \texttt{\small keep\_implicit\_in\_memory} (in the \texttt{\small properties} file) controls whether some {\em implicit} items are stored in memory. The implicit nodes and edges are typically those that cannot be matched to query keyword, e.g. nodes/edges without a label, datasource nodes, etc. During search, these items are mainly used to build answer trees. Storing them in memory can be used either to avoid crowding the underlying database with items, or reduce the cost of reading and writing to disk. One disadvantage of storing implicit items in memory is that they must be reloaded upon every execution, effectively forcing a re-traversal of all the documents.

The entry point for data registration is \href{https://gitlab.inria.fr/cedar/kwd_search_het_code/blob/develop/src/main/java/fr/inria/cedar/connectionlens/ConnectionLens.java#L412}{\texttt{ConnectionLens.register}}. 
The document traversal methods are datasource-specific and implemented by overriding the \href{https://gitlab.inria.fr/cedar/kwd_search_het_code/blob/develop/src/main/java/fr/inria/cedar/connectionlens/source/DataSource.java#L107}{\texttt{DataSource.traverseEdges}} interface method.

~\\
There are \textbf{three ways to turn the nodes of a dataset into CL nodes} 
\begin{description}
\item{\texttt{\small PER\_INSTANCE}} This is the simplest method. It creates as many CL nodes as there are nodes in the data. For instance, if a dataset has 10 people living in Paris (think $p_i\xrightarrow{\text{livesIn}}$ ``Paris'' with $1\leq i \leq 10$) and 5 enterprises locatedIn Paris ($e_j\xrightarrow{\text{locatedIn}}$ ``Paris'' with $1\leq j \leq 5$), there will be 15 ``Paris'' nodes.\\
This loading mode does not apply to RDF datasets, though, because the RDF data model considers that a literal or URI is a single node, regardless of how many times it appears. 
\item{\texttt{\small PER\_TYPE}} This method considers that all the identical constants occurring on the same path from the dataset root should be unified in a single node. For instance, in the above example, there will be 2 nodes: one for the city where 10 people live, and another for the city where 5 companies are located.\\
Note that this supposes that we can identify a path from a dataset root to every node. In RDF, this is not easy to identify, therefore {\texttt{\small PER\_TYPE}} does not work for RDF. More generally, one could imagine a way of understanding which are the equivalent ``Paris'' constants (one could use, e.g., an \href{https://rdfquotient.inria.fr/}{RDFQuotient summary} for that), but this has not been done yet.  Another reason why it does not apply to RDF is that we wished not to contradict the usual RDF data model (see above). 
\item{\texttt{\small PER\_VALUE}} This method creates a single node for every distinct label found in a given dataset, regardless of where it appears.\\
This is how RDF datasets are treated. 
\end{description}

To summarize:
\begin{itemize}
\item For datasets of a hierarchical data model (text, CSV, relational, HTML, JSON), one can get different graphs changing the above options;
\item An RDF dataset is loaded in \texttt{\small PER\_VALUE} mode regardless of what we specify.
\end{itemize}

\vspace{1mm} 
\noindent\textbf{``Do not link'' nodes} 
Sometimes, we find in the data some values on which we do not want connections to be formed:

\begin{itemize}
\item Some text values are used to encode logical {\em nulls} or missing values. Thus, in HATVP data, we encounter {\em néant}, {\em [Données non publiées]} etc. Even though such nodes may appear quite frequently, connecting on them is meaningless, just as in SQL, a null is not equal to another null.
\item In specific applications, connections through some terms may not be desired. For instance, in a database about French people, ``France'' is likely to be so frequent that any connection through it is meaningless. In such applications, the user may chose not forbid the graph from forming such ``hubs'' which (s)he may find useless, or harmful\footnote{An alternative to preventing such a hub from forming, is to let it be and make sure the query algorithm doesn't get trapped inside.}
\end{itemize}

Currently the code allows to specify a set of \texttt{\small do\_not\_link\_labels}: 
\begin{itemize}
\item Any value node found in the data, and whose label is in that set: 
\begin{enumerate}
\item Will be created as a node of a special type (DoNotLinkNode);
\item WIll never be compared with any other node to establish similarity;
\item Will not be analyzed to extract entities inside. 
\end{enumerate}
\item Any entity extracted by Stanford NER or our own extractor, whose label is in the ``do not link'' set, will be silently ignored (no node will be created for it). This is because if we don't ``respect/want'' these nodes, and we don't want to enable connections through them, there is no point in creating them at all. 
\end{itemize}

\vspace{1mm}
\noindent\textbf{More details on indexing} When processing a dataset, we obtain a list of the basic graph edges corresponding to the dataset. Each edge is then sent to a processor, which does the following for each edge that was not already in the graph:

\begin{enumerate}
\item Establish whether the source and/or the target of the edge was already in the graph. 
\item For each node $n$ that was not already in the graph:
\begin{enumerate}
\item Call the Extractor on the label $L$ of the node; this results in a set of pairs (entity node which is an extracted child of $n$, edge between $n$ and the entity child). 
\item For each  $(en, e)$ pair thus obtained:
\begin{itemize}
\item re-enter the above procedure on the edge $e$ (except that we will not attempt to extract again entities from its nodes);
\item then, index $n$ in a way that depends on the chosen indexing method.\\
\item If the method \fbox{\texttt{\small POSTGRES\_FULLTEXT}} is used, \IM{27/2/20: this is what we currently use} we send $L$ to Postgres and let Postgres index it according to its own internal logic. Then, it will be possible to query the index using Postgres' \href{https://www.postgresql.org/docs/9.5/textsearch-tables.html#TEXTSEARCH-TABLES-SEARCH}{full-text search syntax}.
\item If the method \fbox{\texttt{\small LUCENE}} is used, \IM{27/2/2020: we didn't test this thoroughly as we were very satisfied with the one above.} we send $L$ to Lucene and let Lucene index it according to its internal logic. Then, one can search the Lucene index with the desired keywords.
\end{itemize}
Note that in the last two methods (Postgres and Lucene), the whole $L$ is sent for indexing. That means that if $L$ contained an entity, the entity label will be an index term associated both to the entity node and to $n$, its parent. This leads to some form of erroneous (duplicate) indexing, which is corrected at runtime during query answering (see Section~\ref{sec:simple-gam}). 
\end{enumerate} 
\end{enumerate}

\IM{6/4/20 Label normalization should be discussed in this section}

\mysubsection{Treatment of similar nodes}
\label{sec:equiv-nodes}
%Beyond the edges discussed in Section \ref{sec:pb-statement} (each of which connects nodes from the same dataset), we also consider as part of our  graph \textit{same-as edges} either within a common dataset or between different datasets. 

A na\"ive way to represent equivalent and similar nodes in the graph would consist of adding, between each such two nodes, an edge carrying a {\em sameAs} label, with the confidence value $c$. This na\"ive approach has the drawback of storing $O(p^2)$ edges for equivalent $p$ nodes; if the label is very frequent, e.g., ``France'' in a French personnel dataset, this number can quickly explode. 

Instead, we take a more elaborate approach, as follows:

%\begin{enumerate}
%\item 
($i$)~If $n_1,\ldots n_p$ are equivalent nodes (i.e., with equal labels) found {\em in the same} dataset $D$, \IM{27/2/20: the next phrases describe \texttt{\small PER\_VALUE} loading, Section~\ref{sec:loading-details}} we only create {\em one} node with that label, e.g., $n_1$, assuming that historically, this has been the first node with that label encountered when registering $D$. Then, in any edge resulting from $D$, any node  $n_i$ with $1<i\leq p$ is replaced with $n_1$.  This reflects the idea that the same constant in the same dataset typically has the same significance, e.g., in an employee file, a zipcode such as ``91200'', or an email such as ``a@b.org'' appearing multiple times usually mean the same thing. However, this may also introduce some confusions, e.g., if name=''Marie'' and street=''Marie'' appear in different places in a JSON dataset, this is more  a coincidence than a reliable connection. \IM{27/2/20: the next phrases describe \texttt{\small PER\_TYPE} loading, Section~\ref{sec:loading-details}} To avoid such unwanted node unifications, for datasets that are {\em hierarchical (tree-structured)} before this transformation, e.g., JSON or relational, we use the path from the dataset root to each node as a supplementary criterium for deciding when to unify identical-label nodes. Thus, two same-label nodes on the path .employees.employee.address.zipcode are unified into one, whereas nodes on the different paths .employees.employee.name and .employees.employee.address.street (the two ``Marie'' above) are not.  %\IM{27/2/20: there is also \texttt{\small PER\_INSTANCE} loading where we create one node for each piece of data that we encounter.}

%\item 
($ii$)~If $n_1,\ldots,n_p$ are equivalent nodes found {\em in different datasets} $D_1,\ldots,D_k$, we arbitrarily choose one (say, $n_1$, assuming $D_1$ was registered before all the others) and consider it the  {\em representative} of $n_1,n_2,\ldots,n_p$. Thus, we add a column to the $N$ relation storing nodes defined in Section \ref{sec:basicdatastructures}, turning it into $N(ID, type, \lambda, rep)$. This incurs a constant storage overhead for every node, instead of $O(p^2)$ {\em sameAs} edges for each set of $p$ identical-labeled nodes. If $p=1$, i.e., if a node's label is not shared by any other node, the node represents itself. 
%\end{enumerate}

For node pairs that are similar, we store explicitly the {\em sameAs} edges with a confidence value representing the similarity. This is necessary because one cannot infer such an edge if it is not stored. For instance, if $sim(n_1,n_2)=0.85$ and $sim(n_2,n_3)=0.81$, it is generally not possible to infer the value of $sim(n_1,n_3)$; we need to explicitly store the respective {\em sameAs} edge  with the similarity value serving as the confidence $c$.
For instance, in Figure~\ref{fig:example-graph}, {\em sameAs} edges with a confidence of 1.0 are shown between the two nodes labeled{\sf Marrakech}, the three {\sf P. Balkany} nodes etc.; another with confidence 0.85 connects {\sf Central African Republic} to {\sf Centrafrique} (the labels are not identical).  


\mysubsection{Information extraction}
\label{sec:ie-approach}
%To enable interconnecting poorly structured or even unstructured content, we leverage Information Extraction tools to create more nodes (and edges) in $G$ as follows. 
We apply Named Entity Extraction to identify, within text, people, places, or organizations. In our sample graph, this leads to all the {\em blue, round-noded boxes}: each of them is an entity, added in the graph as a child of the text node inside which it was recognized. When an entity, e.g., {\sf P. Balkany}, is recognized in a text node, the keywords contained in the entity name are indexed as labeling the entity (the text node ``transfers'' the keywords to  its entity child). This allows us to return answer trees as meaningful (containing as many entities) as possible to user queries. 
We are currently developing a tool to extract relationships between entities in a given sentence to enrich the graph with more useful connections.  %whose labels carry more information. More generally, other extractions can be applied, e.g., a topic classifier could attach one or several topic (category) nodes from an ontology to a text node that is about those topics etc.; this would further interconnect our graph. %as we did in~\cite{DBLP:journals/pvldb/BonaqueCCGLMMRT16,cao:hal-02269134} etc. Additional information attached to text nodes such as topics/categories could enable to find alternative ways of connecting datasets.


% \mysubsection{Database schema}

% In this section, we present the schema of the relational database used to persistently store the data structures described above.

% ~\\
% The current schema (with some redundancy) is as follows (key attributes underlined): 

% {\it catalog (\underline{id}, type, path)} \par
% {\it wordindex (\underline{word, ds, item}, type)} \par
% {\it labels (\underline{ds, item}, type, label, dsrep, representative, typerep)} \par
% {\it p2b (\underline{ds, origin, bordernode}, origintype, bordernodetype, path, score)} \par

% The {\it wnc} table stores sameAs links with confidence less than 1.
% On each table, Postgres creates by default an index on the primary key attributes. 
% %\CC{Dans {\it labels}, il faudrait un index sur {\it dsrep, representative}; un autre sur {\it label, ds}.} 
% %\CC{Dans  {\it wnc}, il faudrait un index sur {\it db2, node2}.} \IM{Aug 20, 2018: I am assuming these are solved, and I turn them into the affirmative:}
% The {\em labels} table has an index on {\em dsrep, representative} and another one on {\em label, ds}. Finally, the {\em wnc} table has an index on {\em ds2, node2}. 


% \eat{\mysubsection{Paths and distances in the virtual graph}
% \label{sec:dist2border}

% We begin this subsection by specifying notions of path and distances within the virtual graph. 

% \noindent {\em Distance along a path} Let $n_{src}$ and $n_{dest}$ be two nodes in a given dataset. Let $n_{src} \xrightarrow{a_1,c_1} n_1 \xrightarrow{a_2,c_2} \ldots \xrightarrow{a_L,c_L} n_{dest}$ be a path of $L$ successive edges between $n_{src}$ and $n_{dest}$ of length $L$ (keep in mind that each edge can go in either direction, i.e. we consider paths in the general sense of the undirected graph). The $a_i$s are edge labels and the $c_i$s are edge confidences. 
% Then the distance between the nodes $n_{src}$ and $n_{dest}$ along the path $(n_{src}, n_1,\ldots, n_{dest})$ is defined by: 
% $$ d(n_{src}, n_{dest}) = \sum_{i=1}^{L} \frac{1}{c_i} $$

% \noindent {\em Distance between two nodes} There may be many ways to connect two nodes within a same dataset. In this case, the distance between two nodes is defined as the distance between the two nodes along the shortest path.

% To estimate the size of a given answer tree, it may be useful to know the distance between a node that has a match for a query keyword, and the border nodes of its dataset, in order to estimate what distance has to be covered before traversing that $sameAs$ link. We can store this in a relation $Dist2B(DS_{src}, n_{src},b_{src},dist)$ having for each node $n_{src}@DS_{src}$, the distance (number of edges) to the border node $b_{src}@DS_{src}$. Again, in practice, $Dist2B$ can be ordered first by $DS_{src}$, then  by $n_{src}$ and (for instance) by $dist$. One could also extend it into $Dist2B(DS_{src}, n_{src}, b_{src} , DS_{dest}, n_{dest},  dist_{src})$, to also store the possible dataset(s) $DS_{dest}$ to which this border leads. In this extended form, we probably want $Dist2B$ ordered first by $DS_{src}$, then by $DS_{dest}$ etc.

% \noindent {\em Note: approximate distance to border nodes} If the computation of the distance to the border(s) is too long, one can {\em approximate} it with a lower bound of $0$ if the node has a keyword which is in the index, $1$ otherwise, and an upper bound of $d$ (where $d$ is the diameter of the dataset, that is, the length of the longest path). 

% \noindent {\em Note: edge-to-borders distances}  
% Just like we explained above for nodes, we also compute and store distances from graph {\em edges} to borders in $Dist2B$, as query matches may also be found on edges. 

% The above require the ability to find the paths between nodes in each data source. This can be accomplished by computing reachability between nodes starting from both structural edges and sameAs edges. In particular, Postgres has some ability to compute transitive closure\footnote{See \url{https://www.postgresql.org/docs/current/static/queries-with.html}.}.}


% %\RD{I find the condition "...each keyword $k\in \lambda(n_y)$, we search in the index for existing nodes $n_x$ such that $k\in \lambda(n_x)$" too restrictive. \textbf{How will we be able to attempt to link a node with label "N. Sarkozy" and "Nicolas S." where their environments clearly indicate they point to the same person?} We'll never get to check their surroundings based on the first condition to compute SameAs links.}
% %\IM{Indeed we wouldn't be able to (referring to the snippet I put in bold). In principle, it is possible that structured entities are the same even though they don't agree on any attribute name and value... but not likely! More broadly speaking: there exists a vast literature (and even code) on entity matching and linking, Helena has done some, Themis Palpanas from U. Descartes has the JedAI toolkit (http://jedai.scify.org/) etc. The solution sketched above is indeed rather simple. But I would rather not delve into the details very deeply, at least not now; if we want to add more entity matching logic, we have lots to draw from. I'd rather have an end-to-end solution first and improve it afterward.}



==> score.tex <==
\section{Scoring Answer Trees}
\label{sec:score}

We now discuss how to evaluate the quality of an
answer. Section~\ref{sec:generic-score} introduces the general notion
of score on which we base our approach. Section~\ref{sec:specif}
describes one particular metric we attach to edges in order to
instantiate this score, finally Section~\ref{sec:concrete-score}
details the actual score function we used. 

\subsection{Generic score function}
\label{sec:generic-score}
We have configured our problem setting to allow {\em any scoring function}, which enables the use of different scoring schemes fitting the requirements of different users.
As a consequence, this approach allows us to study the interaction of the scoring function with different properties of the graph.
For instance, we are currently investigating the possibility to {\em learn} what makes an answer interesting for a user, so that we may return customized answers to each user.

Given an answer tree $t$ to a query $Q$, we consider a score function consisting of (at least) the following two components: 

\begin{itemize}
\item The {\em matching score} $ms(t)$, which reflects the quality of the answer
  tree, that is, how well its leaves match the query terms.
\item The {\em connection score} $cs(t)$, which reflects the quality of
  the tree connecting the edges. 
  Any formula can be used here, considering the number of edges, the confidence or any other property
attached to edges, or a query-independent property of the nodes, such as their PageRank or betweenness centrality score etc. 
\end{itemize}

The score of $t$ for $Q$, denoted $s(t)$, is computed as a 
combination of the two independent components $ms(t)$ and $cs(t)$. 
Popular combinations functions 
 (a weighted sums, or  product etc.) are monotonous in both
components, however, our framework does not require it. Finally, both $ms(t)$ and $cs(t)$ can be tuned based on a given user's preferences, to
personalize the score, or make them evolve in time through user feedback etc. 

\mysubsection{Edge specificity}\label{sec:specif}
We  now describe a metric on edges, which we used (through the
connection score $cs(t)$) to favor edges that are ``rare'' for both nodes they
connect. This metric was inspired by our experiments with real-world
data sources, and it helped return interesting answer trees in our
experience. %; as stated above, any other metric could be used.

%This metric {\em combines information concerning edges of
%  equivalent nodes}; also an issue is how to {\em compute and maintain it
% efficiently}, as data sets are added to the graph.  We stress that any
% other metric could be used, since our query algorithm does not make
% any assumption about the score. 


For a given node $n$ and label $l$, let $\edgesin{n}{l}$ be the number of $l$-labeled edges entering $n$, and $\edgesout{n}{l}$ the number of $l$-labeled edges exiting $n$. 
\noindent The \textbf{specificity} of an edge $e=n_1\xrightarrow{l}n_2$ is defined as:

\begin{center}
\va\va
$s(e)=2/(\edgesout{n_1}{l} + \edgesin{n_2}{l})$.  
\va\va
\end{center}

$s(e)$ is $1.0$ for edges that are ``unique'' for both their source and their target, and decreases when the edge does not ``stand out'' among the edges of these two nodes.  
For instance,  the city council of Levallois-Perret comprises only one mayor (and one individual cannot be mayor of two cities in France, because he has to inhabit the city where he runs for office). Thus, the edge from the city council to P.~Balkany has a specificity of $2/(1.0+1.0)=1.0$. In contrast, there are 54 countries in Africa (we show only two), and each country is in exactly one continent;  thus,  
the specificity of the {\sf dbo:partOf } edges in the DBPedia fragment, going from the node named Morocco (or the one named Central African Republic) to the node named Africa is $2/(1+54)\simeq .036$. 


\textbf{Specificity computation.}
When  registering the first dataset $D_1$, computing the specificity of its edges is trivial. 
However, when registering subsequent datasets $D_2,D_3$ etc., if some
node, say  $n_2\in D_2$ is found to be equivalent to a node $n_1\in
D_1$,  %both the $D_1$ edges adjacent to $n_1$ and the $D_2$ edges
       %adjacent to $n_2$ are attached to the same conceptual node,
       %representing $n_1,n_2$ and all (possible, future) nodes that
       %are equivalent to them. Therefore, 
{\em all} the $D_1$ edges adjacent to $n_1$ {\em and} the $D_2$ edges adjacent to $n_2$ should be reflected in the specificity of {\em each} of these edges. Thus,  in particular, the specificity of $D_1$ edges needs to be {\em recomputed} when a node in a source added after $D_1$ is equivalent to one of its nodes. 

A {\em na\"ive approach} would be: when the edges of $D_2$ are traversed (when we add this dataset to the graph), re-traverse the edges of $n_1$ in $D_1$ in order to (re)compute their specificity. However, that would be quite inefficient.

Instead, below, we describe an {\em efficient incremental algorithm} to compute specificity. We introduce two notations. 
For any edge $e$, we denote $N^e_{\rightarrow \bullet}$, respectively $N^e_{\circ \rightarrow}$,  the two  numbers out of which the specificity of $e$ has been {\em most recently} computed\footnote{This can be either during the first specificity computation of $e$, or during a recomputation,  as discussed below.}. Specifically,  $N^e_{\rightarrow \bullet}$ counts $l$-labeled edges incoming to the target of $e$, while $N^e_{\circ \rightarrow}$ counts $l$-labeled edges outgoing the source of $e$. In Figure~\ref{fig:edge-recomp}, if $e$ is the edge $x \xrightarrow{l}n_1$, then $N^e_{\rightarrow \bullet}=3$ (blue edges) and $N^e_{\circ \rightarrow}=1$, thus $s(e)=2/4=.5$.  

\begin{figure}[t!]
\begin{center}
\input{images/edge-specif-tikz}
%\vspace{-5mm}
\caption{Illustration for specificity (re)computation. The specificity of the edge $x \xrightarrow{l}n_1$, $s(e)$ is initially computed out of the blue edges; when $n_2$ joins the equivalence set $es_1$, it is recomputed to also reflect the violet edges. \label{fig:edge-recomp}}
\end{center}
\vspace{-7mm}
\end{figure}


Let $n_1\in D_1$ be a node, $es_1$ be the set of all nodes equivalent to
$n_1$, and $n_2\in D_2$ be a node in a dataset we currently register,
and which has just been found to be equivalent to $n_1$, also. 

Further, let $l$ be a label of an edge incoming or outgoing  (any) node from $es_1$, and/or $n_2$.
We denote by $\edgesin{es_1}{l}$ the sum $\sum_{n\in es_1}(\edgesin{n}{l})$  and similarly by $\edgesout{es_1}{l}$ the sum $\sum_{n\in es_1}(\edgesout{n}{l})$; they are the numbers of $l$-labeled outgoing (resp., incoming) $l$-labeled edges of any node in $es_1$. 
When $n_2$ joins the equivalence set $es_1$ of $n_1$ (see Figure~\ref{fig:edge-recomp}): 

\va\va
\begin{enumerate}
\item \label{item:incremental-1}
%\noindent\textbf{1. }
If $\edgesin{es_1}{l}\neq 0$ and $\edgesin{n_2}{l}\neq 0$, the specificity of every $l$-labeled edge $e$  {\em incoming} either a node in $es_1$ or the node $n_2$ must be recomputed.\\
Let $e$ be such an {\em incoming} edge labeled $l$. When $n_2$ is added to the set $es_1$, the specificity of $e$  becomes %: 
%
%\va\va
%\begin{center}
$2/((N^e_{\rightarrow \bullet} + \edgesin{n_2}{l}) + N^e_{\circ \rightarrow})$, 
%\end{center}
%\va\va
%
%\noindent 
to reflect that $n_2$ brings more incoming $l$-labeled edges. This amounts to $2/(3+2+1)=.33$ in Figure~\ref{fig:edge-recomp}: the violet edges have joined the blue ones. Following this adjustment, the numbers out of which $e$'s specificity has been most recently computed are modified as follows: 
%
%\va
%\begin{itemize}
%\item 
$N^e_{\rightarrow \bullet}$  becomes $N^e_{\rightarrow \bullet} + \edgesin{n_2}{l}$, thus $3+2=5$ in Figure~\ref{fig:edge-recomp}; 
%\item 
$N^e_{\circ \rightarrow}$ remains unchanged.
%\end{itemize}
\va
\item \label{item:incremental-2} 
%\noindent\textbf{2. }
If $\edgesin{es_1}{l}=0$ and $\edgesin{n_2}{l}\neq 0$, the specificity of every $l$-labeled edge $e$  {\em incoming} $n_2$ %($es_1$ has no such incoming edges) 
does not change when $n_2$ joins the equivalence set $es_1$. % However, $e$ should be considered as now being adjacent to the equivalence group $es_1$.
%
\item \label{item:incremental-3}
%\noindent\textbf{3. }
If $\edgesin{es_1}{l}\neq 0$ and $\edgesin{n_2}{l}=0$, the newly added node $n_2$ does not change the edges adjacent to the nodes of $es_1$, nor their specificity values.

\printIfExtVersion{
%\item 
\noindent\textbf{4. }
Similarly to \textbf{1.} %\ref{item:incremental-1}. 
above, if $\edgesout{es_1}{l}\neq 0$ and $\edgesout{n_2}{l}\neq 0$, the specificity of every $l$-labeled edge $e$  {\em outgoing} either a node in $es_1$ or the node $n_2$ is recomputed, and it becomes 
%
%\va\va
%\begin{center}
$2/(N^e_{\rightarrow \bullet} + (N^e_{\circ \rightarrow}+\edgesout{n_2}{l}))$. 
%\end{center}
%\va\va
%
The numbers out of which $e$'s specificity has been most recently computed become: $N^e_{\rightarrow \bullet}$  and  $(N^e_{\circ \rightarrow}+\edgesout{n_2}{l})$.
%
%\item 
\noindent\textbf{5. }
Finally, if  $\edgesout{es_1}{l}=0$ and $\edgesout{n_2}{l}\neq 0$, the reasoning is similar to the one in \textbf{2. } %item~2. %(\ref{item:incremental-2}) 
above, while if  $\edgesout{es_1}{l}\neq 0$ and $\edgesout{n_2}{l}=0$, it is similar to \textbf{3.}; %item~3.;%(\ref{item:incremental-3}); 
in both cases, we consider outgoing (instead of incoming) edges and edge count numbers.
}{
\end{enumerate}
\va
The last two cases, when $\edgesout{es_1}{l}\neq 0$ and $\edgesout{n_2}{l}\neq 0$, respectively, $\edgesout{es_1}{l}=0$ and $\edgesout{n_2}{l}\neq 0$, are handled in a similar manner. 
}
%\vspace{2mm}
%Now consider the case of a node $n_3$, similar with confidence $c<1$ to some node $n_1$ whose equivalence class is $es_1$. Node $n_2$ does not join $es_1$. However, when it is found to be $c$-similar to $n_1$, one could follow exactly the procedure described above, by replacing $\edgesin{n_2}{l}$ with $c\cdot \edgesin{n_2}{l}$ and $\edgesout{n_2}{l}$ with $c\cdot \edgesout{n_2}{l}$.

The above method only needs, for a given node $n_2$ newly added to the graph, and label $l$, the number of edges adjacent to $n_2$ in its dataset, and the \emph{number} of $l$ edges  adjacent to a node equivalent to $n_2$. Unlike the na\"ive specificity computation method,  it does not need to actually {\em traverse} these edges previously registered edges, making it more efficient.  

Concretely, for each edge $e\in E$, we store three attributes: $N^e_{\rightarrow \bullet}$, $N^e_{\circ \rightarrow}$  and $s$, the last-computed specificity, and we update $N^e_{\rightarrow \bullet}$, $N^e_{\circ \rightarrow}$ as explained above. 

\begin{comment}	%\ACA{Implementation details, which are not important to give at this point}
\textbf{Where is specificity information stored}
We store a {\it specificity (\underline{representative, edgelabel},
  nIn, nOut)} table. As the specificities are computed jointly for all
the edges adjacent to a set of equivalent nodes, this information is
stored per representative of an equivalence class.  {\it edgeLabel} is
the label of some edge(s) adjacent to this equivalence class; {\it
  nIn} and {\it nOut} are the numbers out of which specificity has
been most recently computed. As an extra optimization, we only store a
tuple in this table if $nIn>1$ or $nOut>1$. Thus, for tree or
tree-like datasets, there are much fewer tuples in the specificity
table than there are in the edges table. 
\end{comment}

\subsection{Concrete score function}
\label{sec:concrete-score}
In our experiments, we used the following score function.


% Formally, let $t=(N,E)$ be an answer tree to a query $Q=\{w_{1},\ldots,w_{n}\}$.

For an answer $t$ to the query $Q$, we compute the matching score $ms(t)$  as the \emph{average}, over all query keywords $w_i$, of the similarity between the $t$ node matching $w_i$ and the keyword $w_i$ itself; we used the edit distance. 
% Similarity is calculated by using any applicable similarity function based on distance measures that are monotonous, thus allowing us to rank the matching entities based on the given similarity measure.

We compute the connection score $cs(t)$ based on edge confidence, on one hand, and edge specificity on the other. We {\em multiply} the confidence values, since we consider that uncertainty (confidence $<1$) multiplies; and we also {\em multiply}  the specificities of all edges in $t$, to discourage many low-specificity edges. Specifically, our score is computed as: 

% The \textbf{connection score} $conns(t)$ is a scalar corresponding to the product of the connectivity associated with every edge of the answer tree: $\prod_{e\in  E} c(e)$. 

% The \textbf{specificity score} $spec(t)$ is similar to the connection score, as we replace connectivity with specificity, and it is computed as: $\prod_{e\in E} s(e)$.

\va\va
\begin{center}
$score(t,Q)=\alpha \cdot ms(t,Q) + \beta \cdot \prod_{e\in  E} c(e) + (1 - \alpha - \beta) \cdot \prod_{e\in E} s(e)$
\end{center}
\va\va

\noindent where $\alpha$, $\beta$ are parameters of the system such that $0\leq \alpha, \beta <1$ and $\alpha +\beta\leq 1$.

\subsection{Orthogonality between the score and the algorithm}

Before we describe the search algorithm, we make a few more remarks on the connection between the score function and the search algorithm. 

We start by considering the classical Steiner Tree and Group Steiner Tree Problems (Section~\ref{sec:steiner}). These assume that the tree cost is \textbf{monotonous}, that is: for any query $Q$ and all trees \textcolor{red}{$T_1, T_2$} where \textcolor{red}{$T_1$} is a subtree of \textcolor{red}{$T_2$}, the cost of \textcolor{red}{$T_2$} is higher  (in our terminology, its score \textcolor{red}{$score(T_2, Q)$} is lower) than that of \textcolor{red}{$T_1$}. This is naturally satisfied if the cost is the addition of edge weights. 
In contrast, % a last difference beween our problem and (G)STP is that:  
% (\pbme)~the 
the score, in its general form  (Section~\ref{sec:generic-score}), and in particular our concrete one  (Section~\ref{sec:concrete-score}), is \textbf{not monotonous}, as illustrated  in Figure~\ref{fig:nonmono}, where on each edge, $c$ is the confidence and $s$ is the specificity. 
% Assume $\alpha=\beta=.5$.
\textcolor{red}{Let} $T$ \textcolor{red}{denote} the four-edge tree rooted in $n_1$, \textcolor{red}{and $T_2$ be the five-edges tree consisting of $T$ plus the edge from $n_4$ to $n_6$.}  Assume $\alpha=\beta=\frac{1}{3}$ and that $T_1,T_2$ have the same matching score.
\textcolor{red}{Then, the last two score terms in $score(T_1,Q)$ are $\frac{1}{3}((.5)^4 + 1)\simeq .35$, while the corresponding terms in $score(T_2,Q)$ are $\frac{1}{3}((.5)^5+.5)\simeq .17$. Thus, $score(T_2,Q)<score(T_1,Q)$, and \textbf{this is not a counterexample to the claimed monotonicity}.}
%the \textcolor{red}{second score componen of $score(T,Q)$ is} $\beta + (1-\alpha-\beta)\cdot (.5)^4$.
%\textcolor{red}{If we denote by $T'$ thee tree while $cs(T')=\beta  \cdot .5 + (1-\alpha-\beta) (.5)^4 \cdot .25$.  If we assume $\alpha=\beta=\frac{1}{3}$,
%then $cs(T)=\frac{1}{3}(1+(.5)^4)\simeq .35$ while $cs(T')=\frac{1}{3}\cdot (.5 + (.5)^5)\simeq .17$, which is clearly smaller. 
%Assuming  $T'$ has the same matching score as $T$, the global score of $T'$ is smaller than that of $T$, contradicting the monotonicity assumption.

\begin{figure*}[t!]
\begin{center}
%\includegraphics[scale=0.6]{images/nonmonotonicity.png}
\tikzstyle{node} = [text centered, fill=white]%blue!30]
\tikzstyle{arrow} = [thick,->,>=stealth]
\begin{tikzpicture}[node distance=34mm and 34mm]% y, then x distance.
\node (zero) {~}; 
\node (n1) [node, right of=zero, xshift=-14mm] {$n_1$};
\node (n2) [node, left of=n1, yshift=4mm] {$n_2$};
\node (n3) [node, left of=n1, yshift=-4mm] {$n_3$};
\node (n4) [node, right of=n1, yshift=4mm] {$n_4$};
\node (n5) [node, right of=n1, yshift=-4mm] {$n_5$};
\draw [arrow] (n1) -> (n2) node [midway, fill=white] {$s=.5,c=1$};
\draw [arrow] (n1) -> (n3) node [midway, fill=white] {$s=.5,c=1$};
\draw [arrow] (n1) -> (n4) node [midway, fill=white] {$s=.5,c=1$};
\draw [arrow] (n1) -> (n5) node [midway, fill=white] {$s=.5,c=1$};
\node (n6) [node, right of=n4] {$n_6$};
\node (n7) [node, right of=n5] {$n_7$};
\draw [arrow, dashed] (n4) -> (n6) node [midway, fill=white] {$s=.25,c=.5$}; % formerly 'f' edge
\draw [arrow, dashed] (n5) -> (n7) node [midway, fill=white] {$s=1,c=1$}; % formerly 'g' edge
\end{tikzpicture}
%$cs(T)=.53125$ \hfill  $cs(T\cup\{n_4\rightarrow n_6\})=.265625$ \hfill $conns(T\cup\{n_5\rightarrow n_7\})=.79$
\caption{Example (non-monotonicity of the tree score). $T$ is the four-edges tree rooted in $n_1$.}
\label{fig:nonmono}
\end{center}
%\vspace{-9mm}
\end{figure*}

% RELATED WORK
% In the literature, (G)STP has been addressed making various simplifying assumptions that do not hold in our context. For instance: the quality of a solution exponentially decreases with the tree size, thus search can stop when all trees are under a certain threshold~\cite{DBLP:conf/edbt/BonaqueCGM16}; edges are considering in a single direction~\cite{DBLP:journals/debu/YuQC10,Elbassuoni:2011:KSO:2063576.2063615,DBLP:journals/tkde/LeLKD14}; 
% the cost function is monotonous~\cite{dpbf} etc. While these assumptions reduce the computational cost, they are all contradicted by concrete examples we encountered while analyzing our journalist partner's datasets. Algorithms which find {\em bounded approximations}, i.e., (G)STP trees solutions whose cost is at most $p$ times higher than the optimal cost, e.g.,~\cite{soda1998,DBLP:conf/cikm/GubichevN12} are not applicable, either: in a data journalism context, journalists want to be the first to uncover an interesting data connection, not one ``at most $p$ times less interesting''. 

Another property sometimes assumed by score functions is the called  \textbf{optimal substructure}, that is: the best solution for a problem of size $p$ is part of the best solution for a problem of size $p+1$ that is an extension of $p$, for some problem size $p$. When this holds, the problem can be efficiently solved in a dynamic programming fashion. 
%% Discussion on optimal substructure (I'm not including it because we're not doing DPBF). If we included it, it would belong *here* because it is a property of the *problem(s)* not of our setting. 
%% 
However, STP  does not enjoy this property: the smallest-cost tree connecting two nodes $n_1,n_2$ is not necessarily part of the smallest-cost tree that connects $n_1,n_2,n_3$ (and the same holds for GSTP). Some existing algorithms also assume a variant of the optimal substructure property (see Section~\ref{sec:related}). In contrast, our score function (both in its general and its concrete form) does not ensure such favorable properties. This is why the search algorithm we describe next has to find as many answers as possible, as quickly as possible. 
% 
%% STP is a particular case of GSTP thus GSTP does not have optimal substructure, either.
%% 
%% DPBF uses "some kind of" optimal substructure for STP as follows: 
%% -- if we have the best way to connect A and B ** through any possible root Rab **
%% -- and the best way to connect B and C through any possible root Rbc
%% -- and the best way to connect A and C through any possible root Rca
%% then ONE OF THESE is part of the best tree connecting A, B and C. 
%% 
%% This relies on the cost function being additive!!! 
%% 
%% Further, DPBF develops all combinations of A, B, C nodes, and solves the STP problem (based on the "kind of" optimal substructure above) for each of them. 
%% Then it returns the best it found. 

% The above search space analysis shows that any connected subtree of $G$ could be part of the answer. Since they cannot be all enumerated, neither can we adopt prior simplifications and restrictions, our approach is to  {\em enumerate $G$ subtrees},  {\em starting from the smallest ones}, in a given {\em time budget}, and striving to find also {\em multi-dataset answers}; when the time budget is exhausted, we return the best $k$ answers found. Enumerating small trees first is both a practical decision (we use them to build larger ones) and fits the intuition that we shouldn't miss small answers that a human could have found manually. Many-dataset answers interest us since they avoid most manual labor to the journalists, by interconnecting multiple data sources, of potentially different formats. 

% \textbf{Lack of monotonicity of the score function.} 
% The score function that we introduce is a linear combination of three parameters: the similarity, the confidence and the specificity.
% All the three parameters are independent with each other and their values depend on the dataset and the query.
% Accordingly, we cannot make any assumptions on their order and, hence, on the monotonicity of the score function.
% Effectively, this means that the score of a given answer tree $T$ may either increase or decrease arbitrarily as we add further nodes and edges to it.
% For instance, adding a node which is an exact match through a weak link (low confidence) may lower the overall score and vice versa: adding a node which is a weak match (low similarity) through a strong link may increase the score. 
% This property is central to our approach, as it provides us with the necessary flexibility to discover solutions which are connected through one or more weak links.  
% Observe that the lack of monotonicity is in fact orthogonal to the existence of the specificity score in the overall score function, as the same argumentation holds for only the matching and the connection score.
% Therefore, our problem cannot be addressed by algorithms considering a monotonic score function, like for instance the (G)STP. 

% \textbf{Lack of optimal substructure of the score function.}
% Consider a query with three keywords.
% It is easy to show that an answer tree which is optimal for matching all the three keywords does not necessarily contain the optimal answer tree for matching only two of the keywords.
% Therefore, we cannot trivially construct a dynamic programming algorithm which solves this problem.
